Single Image Iterative Subject-driven Generation and Editing

Personalizing image generation and editing is particularly challenging when we only have a few images of the subject, or even a single image. A common approach to personalization is concept learning, which can integrate the subject into existing models relatively quickly, but produces images whose quality tends to deteriorate quickly when the number of subject images is small. Quality can be improved by pre-training an encoder, but training restricts generation to the training distribution, and is time consuming. It is still an open hard challenge to personalize image generation and editing from a single image without training. Here, we present SISO, a novel, training-free approach based on optimizing a similarity score with an input subject image. More specifically, SISO iteratively generates images and optimizes the model based on loss of similarity with the given subject image until a satisfactory level of similarity is achieved, allowing plug-and-play optimization to any image generator. We evaluated SISO in two tasks, image editing and image generation, using a diverse data set of personal subjects, and demonstrate significant improvements over existing methods in image quality, subject fidelity, and background preservation.

==> figs/failure.tex <==

\begin{figure}
    \centering
    \scalebox{0.9}{
    \setlength{\tabcolsep}{1pt}
    %\small % This sets the font size for everything inside the figure environment
    \begin{tabular}{cccc }
        & Subject & & Output \\

        \raisebox{26pt}{\rotatebox[origin=t]{90}{\small ... in Versailles}} &
        \includegraphics[width=0.14\linewidth]{images/failure/backpack_ref.jpg} &
                \raisebox{28pt}{$\rightarrow$} &
        \includegraphics[width=0.14\linewidth]{images/failure/backpack_out.jpg} \\
        
        \raisebox{26pt}{\rotatebox[origin=t]{90}{\small ... in the beach}} &
        \includegraphics[width=0.14\linewidth]{images/failure/clock_ref.png} &
                \raisebox{28pt}{$\rightarrow$} &
        \includegraphics[width=0.14\linewidth]{images/failure/clock_out.jpg} \\



    \end{tabular}
    \caption{Failure cases. While the generated backpack's shape is similar to the subject, the color is different and the stickers are missing. In the clock example, the generated images lacks the yellow number three inside the clock.} 
    }
    \label{fig:failure}
    
\end{figure}




==> figs/prompt_simplification.tex <==
% \begin{figure}[t!]
%     \centering
%     \setlength{\tabcolsep}{1pt}
%     \scriptsize{
%     \large
%     \begin{tabular}{cccc}
%         & Subject & Prompt Simplification & w/o Prompt Simplification \\

%         \raisebox{20pt}{\rotatebox[origin=t]{90}{... reading a paper}} &
%         \includegraphics[width=0.2\linewidth]{images/prompt_simplification/sloth_ref.jpg} &
%         \includegraphics[width=0.2\linewidth]{images/prompt_simplification/sloth_w_prompt_simp.jpg} &
%         \includegraphics[width=0.2\linewidth]{images/prompt_simplification/sloth_wo_prompt_simp.jpg} \\

%         \raisebox{20pt}{\rotatebox[origin=t]{90}{... on Coachella}} &
%         \includegraphics[width=0.2\linewidth]{images/prompt_simplification/dog5_ref.jpg} &
%         \includegraphics[width=0.2\linewidth]{images/prompt_simplification/dog5_w_prompt_simp.jpg} &
%         \includegraphics[width=0.2\linewidth]{images/prompt_simplification/dog5_wo_prompt_simp.jpg} \\

%    \end{tabular}
%     }
%     \caption{
%         We show the stability of our method across multiple seed
%     }
%     \label{fig:prompt_simp}
% \end{figure}


==> figs/reuse.tex <==
\begin{figure}
    \centering
    \setlength{\tabcolsep}{1pt}
    \scriptsize{
    \begin{tabular}{c c ccc}
        Input & Optimized & \multicolumn{3}{c}{Reuse Optimized Weights} \\
        \includegraphics[width=0.20\linewidth]{images/reuse/cat_ref.png} &
        \includegraphics[width=0.20\linewidth]{images/reuse/cat_optim.png} &
        \includegraphics[width=0.20\linewidth]{images/reuse/cat_wine.png} &
        \includegraphics[width=0.20\linewidth]{images/reuse/cat_beach.png} &
        \includegraphics[width=0.20\linewidth]{images/reuse/cat_sleep.png} 
        \\
        & a photo of a ... & ... drinking wine & ... in the beach & ... sleeping \\

        \includegraphics[width=0.20\linewidth]{images/reuse/chair_ref.png} &
        \includegraphics[width=0.20\linewidth]{images/reuse/chair_optim.png} &
        \includegraphics[width=0.20\linewidth]{images/reuse/chair_kitchen.png} &
        \includegraphics[width=0.20\linewidth]{images/reuse/chair_bedroom.png} &
        \includegraphics[width=0.20\linewidth]{images/reuse/chair_living.png} 
        \\
        & a photo of a ... & ... in a kitchen & ... in a bedroom & ... in a living room \\
        
        
    \end{tabular}
    \vspace{-6pt}
    }
    \caption{
    Showcase of the Prompt Simplification 
    }
    \vspace{-10pt}
    \label{fig:reuse}
\end{figure}


==> figs/subject_stability.tex <==
\begin{figure*}[t!]
    \centering
    \setlength{\tabcolsep}{1pt}
    \scriptsize{
    \large
    \begin{tabular}{cccccccc}
        Input Image & & Subject & Output & Subject & Output & Subject & Output \\

        \includegraphics[width=0.13\linewidth]{images/subject_stability/cat_bg.jpeg} &
        \raisebox{28pt}{$\rightarrow$} &
        \includegraphics[width=0.13\linewidth]{images/subject_stability/cat_ref.png} &
        \includegraphics[width=0.13\linewidth]{images/subject_stability/cat_out.jpeg} &
        \includegraphics[width=0.13\linewidth]{images/subject_stability/cat2_ref.png} &
        \includegraphics[width=0.13\linewidth]{images/subject_stability/cat2_out.jpeg} &
        \includegraphics[width=0.13\linewidth]{images/subject_stability/cat5_ref.png} &
        \includegraphics[width=0.13\linewidth]{images/subject_stability/cat5_out.jpeg} \\
        
        \end{tabular}
    }
    \caption{
        We show that our method can edit the same input images with multiple subjects
    }
    \label{fig:subject_stability}
\end{figure*}



